Directed Reachability for Infinite-State Systems

Numerous tasks in program analysis and synthesis reduce to deciding reachability in possibly infinite graphs such as those induced by Petri nets. However, the Petri net reachability problem has recently been shown to require non-elementary time, which raises questions about the practical applicability of Petri nets as target models. In this paper, we introduce a novel approach for efficiently semi-deciding the reachability problem for Petri nets in practice. Our key insight is that computationally lightweight over-approximations of Petri nets can be used as distance oracles in classical graph exploration algorithms such as A* and greedy best-first search. We provide and evaluate a prototype implementation of our approach that outperforms existing state-of-the-art tools, sometimes by orders of magnitude, and which is also competitive with domain-specific tools on benchmarks coming from program synthesis and concurrent program analysis.

==> benchmark-figs/fig-gbfs-comparisons.tex <==
\begin{figure}[h]
  \centering
  \begin{minipage}[t]{0.31\textwidth}%
    \centering
    \input{benchmark-figs/fig-gbfs-comparison-gbfs.tex}%
  \end{minipage}%
  \begin{minipage}[t]{0.31\textwidth}%
    \centering
    \input{benchmark-figs/fig-gbfs-comparison-dijkstra.tex}%
  \end{minipage}%
  \begin{minipage}[t]{0.31\textwidth}%
    \centering
    \input{benchmark-figs/fig-gbfs-comparison-lola.tex}%
  \end{minipage}%
  
  \begin{minipage}[t]{0.31\textwidth}%
    \centering
    \input{benchmark-figs/fig-gbfs-comparison-bfc.tex}%
  \end{minipage}%
  \begin{minipage}[t]{0.31\textwidth}%
    \centering
    \input{benchmark-figs/fig-gbfs-comparison-icover.tex}%
  \end{minipage}%
  \begin{minipage}[t]{0.31\textwidth}%
    \centering
    \input{benchmark-figs/fig-gbfs-comparison-mist.tex}%
  \end{minipage}%
\caption{Runtime comparison against \textsc{FF(GBFS,
    $\mathcal{D}_{\Q}$)}, in seconds, for individual instances without
  pre-pruning. Tools on the first row include coverability and
  reachability instances, others only include coverability. Marks on
  the \textcolor{gray!80!black}{gray} lines denote timeouts
  ($60$~s).}\label{fig:comparisons}
%% \caption{Runtime comparison against \textsc{FF(\astar, $\mathcal{D}_{\Q}$)} in seconds for individual instances without pre-pruning. Comparisons with \textsc{LoLA} and \textsc{FF(\astar, $0$)} include coverability and reachability instances, others only include coverability. \textcolor{red}{Red x}'s denote negative instances, \textcolor{blue}{blue crosses (+)} denote positive ones. Marks on the \textcolor{gray!80!black}{gray} lines denote timeouts ($60$ s).}\label{fig:comparisons}
\end{figure}


==> benchmark-figs/fig-heuristics.tex <==
\begin{figure}[!h]
    \centering
\heuristicplot{shortest path length}{initial heuristic value}{

    \addplot[] plot coordinates {(0,0) (50, 50)};

    % N Marking equation
    \addplot[only marks, mark=triangle*, color=colFastForward NMarkingEQGurobi+Pruning+Competitive, mark size=3 pt] plot coordinates {(13, 13) (67, 67) (10, 10) (4, 4) (32, 32) (28, 28) (50, 50) (25, 25) (50, 50) (28, 28) (34, 34) (34, 34) (28, 28) (28, 28) (30, 30) (40, 40) (30, 30) (28, 28) (34, 34) (50, 50) (28, 28) (50, 50) (28, 28) (40, 40) (25, 25) (15, 14) (22, 20) (15, 14) (21, 20) (22, 20) (15, 14) (1, 1) (2, 2) (3, 3) (4, 4) (4, 2) (2, 2) (2, 2) (3, 2) (3, 3) (4, 4) (3, 3) (2, 2) (2, 2) (5, 4) (1, 1) (2, 2) (3, 3) (2, 2) (2, 2) (2, 1) (3, 3) (1, 1) (4, 2) (4, 4) (3, 2) (3, 2) (2, 2) (1, 1) (17, 13) (14, 6) (11, 9) (8, 8) (9, 6) (21, 19) (14, 14) (11, 8) (8, 8) (17, 11) (13, 10) (16, 16) (31, 24) (18, 14) (22, 10) (21, 17) (14, 14) (13, 13) (12, 12) (11, 6) (12, 9) (13, 7) (9, 9) (30, 25) (23, 21) (11, 8) (22, 10) (11, 6) (8, 6) (40, 33) (26, 23) (22, 21) (19, 11) (12, 9) (10, 10)};

    % Q Marking equation
    \addplot [only marks, mark=diamond*, color=colFastForward QMarkingEQGurobi+Pruning+Competitive, mark size=2pt] plot coordinates {(16, 16) (4, 4) (10, 10) (7, 7) (8, 8) (11, 11) (11, 11) (11, 11) (12, 12) (5, 5) (13, 13) (17, 17) (5, 5) (4, 4) (4, 4) (19, 19) (28, 28) (10, 10) (8, 8) (7, 7) (6, 6) (5, 5) (8, 8) (7, 7) (4, 4) (5, 5) (2, 2) (22, 22) (9, 9) (7, 7) (6, 6) (7, 7) (11, 11) (50, 50) (8, 8) (6, 6) (17, 17) (10, 10) (15, 15) (15, 15) (14, 14) (14, 14) (20, 20) (17, 17) (11, 11) (16, 16) (5, 5) (11, 11) (11, 11) (13, 13) (5, 5) (15, 15) (29, 29) (7, 7) (10, 10) (5, 5) (5, 5) (11, 11) (16, 16) (11, 11) (7, 7) (4, 4) (16, 16) (5, 5) (11, 11) (5, 5) (15, 15) (16, 16) (4, 4) (7, 7) (4, 4) (6, 6) (5, 5) (25, 25) (10, 10) (2, 2) (5, 5) (17, 17) (22, 22) (25, 25) (15, 15) (16, 16) (10, 10) (15, 15) (2, 2) (50, 50) (22, 22) (10, 10) (15, 15) (5, 5) (19, 19) (15, 15) (28, 28) (7, 7) (34, 34) (3, 3) (5, 5) (34, 34) (22, 22) (24, 24) (13, 13) (7, 7) (11, 11) (14, 14) (20, 20) (24, 24) (5, 5) (5, 5) (7, 7) (8, 8) (28, 28) (7, 7) (5, 5) (16, 16) (8, 8) (10, 10) (18, 18) (5, 5) (15, 15) (16, 16) (17, 17) (16, 16) (11, 11) (17, 17) (11, 11) (17, 17) (9, 9) (7, 7) (17, 17) (5, 5) (5, 5) (4, 4) (4, 4) (12, 12) (17, 17) (9, 9) (12, 12) (4, 4) (21, 21) (8, 8) (6, 6) (4, 4) (28, 28) (30, 30) (16, 16) (23, 23) (7, 7) (7, 7) (4, 4) (16, 16) (20, 20) (17, 17) (15, 15) (7, 7) (7, 7) (22, 22) (20, 20) (4, 4) (11, 11) (40, 40) (6, 6) (12, 12) (15, 15) (9, 9) (16, 16) (4, 4) (4, 4) (11, 11) (12, 12) (22, 22) (30, 30) (17, 17) (8, 8) (4, 4) (7, 7) (9, 9) (12, 12) (5, 5) (5, 5) (4, 4) (20, 20) (17, 17) (4, 4) (11, 11) (3, 3) (5, 5) (7, 7) (4, 4) (11, 11) (4, 4) (12, 12) (6, 6) (18, 18) (4, 4) (28, 28) (10, 10) (20, 20) (5, 5) (6, 6) (5, 5) (8, 8) (7, 7) (12, 12) (5, 5) (9, 9) (7, 7) (12, 12) (5, 5) (7, 7) (4, 4) (17, 17) (11, 11) (7, 7) (10, 10) (10, 10) (16, 16) (11, 11) (10, 10) (7, 7) (3, 3) (4, 4) (16, 16) (8, 8) (6, 6) (5, 5) (34, 34) (12, 12) (22, 22) (14, 14) (5, 5) (4, 4) (6, 6) (4, 4) (50, 50) (7, 7) (1, 1) (2, 2) (3, 2) (4, 4) (4, 2) (2, 2) (2, 2) (3, 2) (3, 2) (4, 3) (3, 3) (2, 2) (2, 2) (5, 3) (1, 1) (2, 2) (3, 2) (2, 2) (2, 2) (2, 1) (3, 2) (1, 1) (4, 2) (4, 4) (3, 2) (3, 2) (2, 2) (1, 1) (15, 11) (11, 8) (8, 8) (12, 8) (12, 8) (17, 11) (17, 9) (16, 16) (19, 9) (18, 10) (14, 14) (13, 13) (30, 25) (18, 10) (36, 33) (26, 23) (22, 21) (17, 11) (12, 9)};

    % Q Reachability
    \addplot [only marks, mark=x, color=colqreach, mark size = 1pt] plot coordinates {(67, 67) (10, 10) (4, 4) (32, 32) (28, 28) (25, 25) (34, 34) (34, 34) (28, 28) (30, 30) (40, 40) (30, 30) (34, 34) (28, 28) (25, 25) (15, 15) (22, 21) (15, 15) (21, 21) (22, 21) (15, 15) (1, 1) (2, 2) (3, 2) (4, 3) (4, 4) (2, 2) (2, 2) (3, 4) (4, 3) (2, 2) (2, 2) (5, 4) (1, 1) (2, 2) (3, 6) (2, 2) (2, 2) (3, 2) (1, 1) (4, 2) (4, 4) (3, 3) (3, 3) (2, 2) (1, 1) (17, 12) (11, 11) (8, 8) (9, 9) (21, 21) (14, 14) (11, 6) (8, 8) (17, 17) (13, 13) (16, 16) (31, 29) (14, 14) (13, 13) (12, 12) (11, 11) (12, 12) (9, 9) (30, 28) (11, 7) (11, 11) (8, 8) (26, 26) (22, 22) (19, 15) (12, 12) (10, 10)};

    % syntactic
    \addplot [only marks, mark=+, color=colsyntactic, mark size = 1pt] plot coordinates {(13, 0) (67, 0) (10, 0) (4, 0) (32, 0) (28, 1) (50, 1) (25, 2) (50, 2) (28, 1) (34, 1) (34, 1) (28, 1) (28, 1) (30, 2) (40, 1) (30, 1) (28, 1) (34, 1) (50, 2) (28, 1) (50, 2) (28, 2) (40, 1) (25, 2) (15, 0) (22, 0) (15, 0) (21, 0) (22, 0) (15, 0) (1, 1) (2, 1) (3, 1) (4, 1) (4, 1) (2, 1) (2, 1) (3, 1) (3, 1) (4, 1) (3, 1) (2, 1) (2, 1) (5, 1) (1, 0) (2, 1) (3, 1) (2, 1) (2, 1) (2, 0) (3, 1) (1, 0) (4, 1) (4, 1) (3, 1) (3, 1) (2, 1) (1, 0) (17, 0) (14, 0) (11, 0) (8, 0) (9, 0) (21, 0) (14, 0) (11, 0) (8, 0) (17, 0) (13, 0) (16, 0) (31, 0) (18, 0) (22, 0) (21, 0) (14, 0) (13, 0) (12, 0) (11, 0) (12, 0) (13, 0) (9, 0) (30, 0) (23, 0) (11, 0) (22, 0) (11, 0) (8, 0) (40, 0) (26, 0) (22, 0) (19, 0) (12, 0) (10, 0)};
}

\begin{tikzpicture}[very thick, scale=\plotscale,
    every node/.style={scale=\plotscale}]
\begin{customlegend}[legend columns=4,
legend style={draw=none, column sep=1ex},
legend entries={
\textsc{$\mathcal{D}_\Z$},
\textsc{$\mathcal{D}_\Q$},
\textsc{$\mathcal{D}_{\Q_{+}}$},
\textsc{$d_{struct}$}}] 
\addlegendmark{FastForward NMarkingEQGurobi+Pruning+Competitive}{triangle*}
\addlegendmark{FastForward QMarkingEQGurobi+Pruning+Competitive}{diamond*}
\addlegendmark{qreach}{x}
\addlegendmark{syntactic}{+}
\end{customlegend}
\end{tikzpicture}

\caption{Initial heuristic estimation compared to the length of a shortest witness. Points closer to the diagonal indicate better estimations.}
\end{figure}


==> benchmark-figs/fig-pruning.tex <==
\begin{figure}[h]
    \begin{minipage}[t]{0.48\textwidth}
      \input{benchmark-figs/fig-pruning-places.tex}
    \end{minipage}%
    \hspace*{15pt}
    \begin{minipage}[t]{0.48\textwidth}
      \input{benchmark-figs/fig-pruning-transitions.tex}
    \end{minipage}
  \caption{A plot detailing on how many instances what percentage of
    places (left) and transitions (right) was removed by pruning
    (rounded to the nearest multiple of~10).}\label{fig:coverability}
\end{figure} 


==> benchmark-figs/fig-reachability.tex <==
\begin{figure}[h]
    \begin{minipage}[t]{0.47\textwidth}%
      \input{benchmark-figs/fig-reachability-not-prepruned.tex}
    \end{minipage}%
    \hspace*{5pt}%
    \begin{minipage}[t]{0.47\textwidth}%
      \input{benchmark-figs/fig-reachability-prepruned.tex}
    \end{minipage}%
        %% Bottom legend
        \begin{center}
        \begin{tikzpicture}[very thick, scale=\plotscale,
          every node/.style={scale=\plotscale}]
  \begin{customlegend}[legend columns=4,
  legend style={draw=none, column sep=1ex},
  legend entries={
  \textsc{FF(\astar, $\mathcal{D}_{\Q}$)},
  \textsc{FF(GBFS, $\mathcal{D}_{\Q}$)},
  \textsc{FF(Dijkstra)},
  \textsc{LoLA}},]
  \addlegend{FastForward QMarkingEQGurobi+Competitive}{diamond*}
  \addlegend{GBFS}{square*}
  \addlegend{FastForward zero+Competitive}{*}
  \addlegend{Lola}{+}
  \end{customlegend}
  \end{tikzpicture}
  \end{center}
  \caption{Cumulative number of \textsc{random-walk} instances decided over
    time. \emph{Left}: Evaluation on the original
    instances. \emph{Right}: Evaluation on the pre-pruned
    instances.}\label{fig:random-walk}
  \end{figure}
  


==> benchmark-figs/fig-sypet.tex <==
\begin{figure}[h]
    \begin{minipage}[t]{0.47\textwidth}%
      \input{benchmark-figs/fig-sypet-not-prepruned.tex}
    \end{minipage}%
    \hspace*{5pt}%
    \begin{minipage}[t]{0.47\textwidth}%
      \input{benchmark-figs/fig-sypet-prepruned.tex}
    \end{minipage}%
        %% Bottom legend
        \begin{center}
        \begin{tikzpicture}[very thick, scale=\plotscale,
          every node/.style={scale=\plotscale}]
  \begin{customlegend}[legend columns=4,
  legend style={draw=none, column sep=1ex},
  legend entries={
  \textsc{FF(\astar, $\mathcal{D}_{\Q}$)},
  \textsc{FF(GBFS, $\mathcal{D}_{\Q}$)},
  \textsc{FF(Dijkstra)},
  \textsc{LoLA}},]
  \addlegend{FastForward QMarkingEQGurobi+Competitive}{diamond*}
  \addlegend{GBFS}{square*}
  \addlegend{FastForward zero+Competitive}{*}
  \addlegend{Lola}{+}
  \end{customlegend}
  \end{tikzpicture}
  \end{center}
  \caption{Cumulative number of \textsc{sypet} instances decided over
    time. \emph{Left}: Evaluation on the original
    instances. \emph{Right}: Evaluation on the pre-pruned
    instances.}\label{fig:sypet}
  \end{figure}
  


==> fig-control-flow-bluetooth.tex <==
\begin{minipage}[t]{0.46\textwidth}
  \lstinputlisting[language=python]{bluetooth_add.py}
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.46\textwidth}
  \lstinputlisting[language=python]{bluetooth_stop.py}
\end{minipage}


==> fig-graphs.tex <==
\begin{figure}[h]
  \begin{center}
    %% Left plot
    \plotcanvas{%
      time $t$ in seconds}{%
      number of instances proven \\ safe in $\leq t$ secs.}{%
      
      %% Petrinizer    
      \toolplot{2}{triangle*}{ (1, 39) (2, 50) (4, 58) (8, 60) (16, 61)
        (32, 62) (64, 95) (2000, 95) };
      
      %% Bfc
      \toolplot{4}{diamond*}{ (1, 33) (2, 37) (4, 38) (8, 41) (16, 42)
        (64, 43) (128, 63) (2000, 63) };
      
      %% Mist (backward)
      \toolplot{3}{square*}{ (1, 18) (2, 20) (4, 21) (8, 25) (16, 29)
        (32, 31) (64, 32) (256, 33) (512, 34) (2000, 35) };
      
      %% QCover
      \toolplot{1}{*}{(1, 50) (2, 53) (4, 59) (8, 63) (16, 90) (32, 96)
        (64, 103) (256, 104) (2000, 105)};
    }%
    %
    \hspace{20pt}
    %
    %% Right plot
    \plotcanvas{%
      time $t$ in seconds}{%
      number of instances proven \\ safe or unsafe in $\leq t$ secs.}{%

      %% Petrinizer
      \toolplot{2}{triangle*}{ (1, 39) (2, 50) (4, 58) (8, 60) (16,
        61) (32, 62) (64, 95) (2000, 95) };

      %% Bfc
      \toolplot{4}{diamond*}{ (1, 81) (2, 87) (4, 89) (8, 94) (16, 97)
        (32, 98) (64, 99) (128, 120) (512, 121) (2000, 122) };

      %% Mist (backward)
      \toolplot{3}{square*}{ (1, 34) (2, 41) (4, 44) (8, 50) (16, 55)
        (32, 57) (64, 63) (256, 67) (512, 69) (2000, 74) };

      %% QCover
      \toolplot{1}{*}{ (1, 53) (2, 57) (4, 70) (8, 77) (16, 108) (32,
        116) (64, 125) (128, 127) (256, 131) (512, 135) (2000, 142) };
    }
    %% Bottom legend
    \begin{tikzpicture}[very thick, scale=\plotscale,
                        every node/.style={scale=\plotscale}]
      \begin{customlegend}[legend columns=-1,
          legend style={draw=none, column sep=1ex},
          legend entries={\textsc{QCover}, \textsc{Petrinizer},
                          \textsc{Bfc},    \textsc{mist}}]
        \addlegend{1}{*}
        \addlegend{2}{triangle*}
        \addlegend{3}{diamond*}
        \addlegend{4}{square*}
      \end{customlegend}
    \end{tikzpicture}
  \end{center}
  \caption{Cumulative number of instances proven safe (left) and total
    number of instances decided (right) within a fixed amount of
    time.}\label{fig:graphs}
\end{figure}


==> fig-medical.tex <==

\begin{figure}[h]
  \begin{center}
    \plotcanvas{%
      time $t$ in deciseconds}{%
      number of instances proven \\ safe in $\leq t$ deciseconds.}{%

      
%% BFC
\toolplot{BFC}{asterisk}{(1, 0)(64, 3)(6000, 3)}{6000}{3}{3/12};


%% a-star+QMarkingEQGurobi+Pruning
\toolplot{a-star+QMarkingEQGurobi+Pruning}{square*}{(1, 0)(4, 10)(6000, 10)}{6000}{10}{10/12};


%% a-star+QMarkingEQGurobi
\toolplot{a-star+QMarkingEQGurobi}{square}{(1, 0)(8, 4)(6000, 4)}{6000}{4}{4/12};


%% a-star+NMarkingEQGurobi+Pruning
\toolplot{a-star+NMarkingEQGurobi+Pruning}{triangle*}{(1, 0)(4, 10)(6000, 10)}{6000}{10}{};


%% a-star+structuralperplace-n+Pruning
\toolplot{a-star+structuralperplace-n+Pruning}{diamond*}{(1, 0)(4, 10)(6000, 10)}{6000}{10}{};


%% best-first+QMarkingEQGurobi+Pruning
\toolplot{best-first+QMarkingEQGurobi+Pruning}{oplus*}{(1, 0)(4, 10)(6000, 10)}{6000}{10}{};


%% best-first+QMarkingEQGurobi
\toolplot{best-first+QMarkingEQGurobi}{oplus}{(1, 0)(8, 4)(6000, 4)}{6000}{4}{};


%% best-first+NMarkingEQGurobi+Pruning
\toolplot{best-first+NMarkingEQGurobi+Pruning}{otimes*}{(1, 0)(4, 10)(6000, 10)}{6000}{10}{};


%% best-first+structuralperplace-n+Pruning
\toolplot{best-first+structuralperplace-n+Pruning}{*}{(1, 0)(4, 10)(6000, 10)}{6000}{10}{};


%% Lola
\toolplot{Lola}{+}{(1, 0)(4, 1)(8, 3)(6000, 3)}{6000}{3}{};


%% QCover
\toolplot{QCover}{star}{(1, 0)(32, 4)(256, 10)(6000, 10)}{6000}{10}{};


%% MIST-Backward
\toolplot{MIST-Backward}{x}{(1, 0)(64, 4)(128, 7)(256, 9)(512, 10)(4096, 11)(6000, 11)}{6000}{11}{11/12};
    }
    %% Bottom legend
    \begin{tikzpicture}[very thick, scale=\plotscale,
                        every node/.style={scale=\plotscale}]
      \begin{customlegend}[legend columns=1,
          legend style={draw=none, column sep=1ex},
          legend entries={\textsc{BFC}, \textsc{a-star+QMarkingEQGurobi+Pruning}, \textsc{a-star+QMarkingEQGurobi}, \textsc{a-star+NMarkingEQGurobi+Pruning}, \textsc{a-star+structuralperplace-n+Pruning}, \textsc{best-first+QMarkingEQGurobi+Pruning}, \textsc{best-first+QMarkingEQGurobi}, \textsc{best-first+NMarkingEQGurobi+Pruning}, \textsc{best-first+structuralperplace-n+Pruning}, \textsc{Lola}, \textsc{QCover}, \textsc{MIST-Backward}}]
        \addlegend{BFC}{asterisk}
\addlegend{a-star+QMarkingEQGurobi+Pruning}{square*}
\addlegend{a-star+QMarkingEQGurobi}{square}
\addlegend{a-star+NMarkingEQGurobi+Pruning}{triangle*}
\addlegend{a-star+structuralperplace-n+Pruning}{diamond*}
\addlegend{best-first+QMarkingEQGurobi+Pruning}{oplus*}
\addlegend{best-first+QMarkingEQGurobi}{oplus}
\addlegend{best-first+NMarkingEQGurobi+Pruning}{otimes*}
\addlegend{best-first+structuralperplace-n+Pruning}{*}
\addlegend{Lola}{+}
\addlegend{QCover}{star}
\addlegend{MIST-Backward}{x}
      \end{customlegend}
    \end{tikzpicture}
  \end{center}
  \caption{Cumulative number of instances decided.}\label{fig:graphs}
\end{figure}
        


==> fig-soter.tex <==

\begin{figure}[h]
  \begin{center}
    \plotcanvas{%
      time $t$ in deciseconds}{%
      number of instances proven \\ safe in $\leq t$ deciseconds.}{%

      
%% BFC
\toolplot{BFC}{asterisk}{(1, 17)(4, 18)(8, 20)(32, 21)(1024, 22)(6000, 22)}{6000}{22}{22/38};


%% QCover
\toolplot{QCover}{star}{(1, 0)(4, 11)(8, 21)(16, 27)(32, 29)(64, 31)(256, 32)(512, 35)(6000, 35)}{6000}{35}{35/38};


%% MIST-Backward
\toolplot{MIST-Backward}{x}{(1, 3)(16, 4)(256, 6)(6000, 6)}{6000}{6}{6/38};


%% a-star+QMarkingEQGurobi+Pruning
\toolplot{a-star+QMarkingEQGurobi+Pruning}{square*}{(1, 0)(2, 1)(4, 23)(8, 26)(32, 27)(128, 28)(256, 29)(512, 30)(2048, 31)(6000, 31)}{6000}{31}{31/38};


%% a-star+QMarkingEQGurobi
\toolplot{a-star+QMarkingEQGurobi}{square}{(1, 0)(2, 8)(4, 22)(8, 25)(16, 27)(256, 29)(1024, 30)(4096, 31)(6000, 31)}{6000}{31}{};


%% a-star+NMarkingEQGurobi+Pruning
\toolplot{a-star+NMarkingEQGurobi+Pruning}{triangle*}{(1, 0)(2, 4)(4, 23)(8, 26)(32, 27)(128, 28)(256, 29)(2048, 30)(6000, 30)}{6000}{30}{30/38};


%% a-star+structuralperplace-n+Pruning
\toolplot{a-star+structuralperplace-n+Pruning}{diamond*}{(1, 0)(4, 23)(8, 25)(16, 26)(32, 27)(128, 28)(512, 29)(2048, 30)(6000, 30)}{6000}{30}{};


%% best-first+QMarkingEQGurobi+Pruning
\toolplot{best-first+QMarkingEQGurobi+Pruning}{oplus*}{(1, 0)(2, 4)(4, 22)(8, 24)(32, 25)(128, 26)(256, 27)(6000, 27)}{6000}{27}{27/38};


%% best-first+QMarkingEQGurobi
\toolplot{best-first+QMarkingEQGurobi}{oplus}{(1, 0)(2, 9)(4, 21)(8, 23)(16, 25)(256, 27)(6000, 27)}{6000}{27}{};


%% best-first+NMarkingEQGurobi+Pruning
\toolplot{best-first+NMarkingEQGurobi+Pruning}{otimes*}{(1, 0)(2, 4)(4, 23)(8, 25)(32, 26)(128, 27)(256, 28)(6000, 28)}{6000}{28}{28/38};


%% best-first+structuralperplace-n+Pruning
\toolplot{best-first+structuralperplace-n+Pruning}{*}{(1, 0)(4, 19)(8, 20)(16, 21)(32, 22)(128, 23)(512, 24)(6000, 24)}{6000}{24}{24/38};


%% Lola
\toolplot{Lola}{+}{(1, 3)(4, 7)(8, 9)(16, 10)(128, 11)(256, 12)(512, 13)(1024, 16)(2048, 21)(4096, 24)(6000, 24)}{6000}{24}{};


    }
    %% Bottom legend
    \begin{tikzpicture}[very thick, scale=\plotscale,
                        every node/.style={scale=\plotscale}]
      \begin{customlegend}[legend columns=1,
          legend style={draw=none, column sep=1ex},
          legend entries={\textsc{BFC}, \textsc{QCover}, \textsc{MIST-Backward}, \textsc{a-star+QMarkingEQGurobi+Pruning}, \textsc{a-star+QMarkingEQGurobi}, \textsc{a-star+NMarkingEQGurobi+Pruning}, \textsc{a-star+structuralperplace-n+Pruning}, \textsc{best-first+QMarkingEQGurobi+Pruning}, \textsc{best-first+QMarkingEQGurobi}, \textsc{best-first+NMarkingEQGurobi+Pruning}, \textsc{best-first+structuralperplace-n+Pruning}, \textsc{Lola}}]
        \addlegend{BFC}{asterisk}
\addlegend{QCover}{star}
\addlegend{MIST-Backward}{x}
\addlegend{a-star+QMarkingEQGurobi+Pruning}{square*}
\addlegend{a-star+QMarkingEQGurobi}{square}
\addlegend{a-star+NMarkingEQGurobi+Pruning}{triangle*}
\addlegend{a-star+structuralperplace-n+Pruning}{diamond*}
\addlegend{best-first+QMarkingEQGurobi+Pruning}{oplus*}
\addlegend{best-first+QMarkingEQGurobi}{oplus}
\addlegend{best-first+NMarkingEQGurobi+Pruning}{otimes*}
\addlegend{best-first+structuralperplace-n+Pruning}{*}
\addlegend{Lola}{+}
      \end{customlegend}
    \end{tikzpicture}
  \end{center}
  \caption{Cumulative number of instances decided.}\label{fig:graphs}
\end{figure}
        


==> ssec-coverability.tex <==
%% \begin{itemize}
%% \item \emph{wahl-kroening}: 44 coverable and 2 uncoverable instances
%%   arising from the analysis of multi-threaded \textsc{C} programs with
%%   shared-memory (used by the tool \textsc{Bfc}~\cite{KKW14}); 
      
%% \item \emph{mist}: 4 coverable and 23 uncoverable instances modeling
%%   various systems such as mutual exclusion algorithms and
%%   communication protocols (used by the tool \textsc{mist}~\cite{P02});
      
%% \item \emph{medical}: 12 uncoverable instances modeling provenance
%%   analysis for a medical messaging system~\cite{BMDS07};
      
%% \item \emph{bug\_tracking}: 1 coverable and 40 uncoverable instances
%%   modeling provenance analysis for a bug-tracking system~\cite{J09};
      
%% \item \emph{soter}: 12 coverable and 38 uncoverable instances arising
%%   from the verification of \textsc{Erlang} concurrent programs (used
%%   by the tool \textsc{SOTER}~\cite{DKO13}).
%% \end{itemize}

\subsection{Reachability towards upward-closed sets (coverability)}

%% \paragraph*{Instances proven.}

%% \Cref{fig:coverability} shows the cumulative number of  instances proven coverable and uncoverable. On the latter, \textsc{FastForward} with \astar\ and with GBFS have near identical performance, so their lines overlap.
%% %
%% For coverable instances, using \textsc{FastForward} with \astar\ and $\mathcal{D}_{\Q}$, we exhibit a witness for \emph{all} 61 instances within the time limit. To our knowledge, no tool was previously able to decide all coverable instances, even with much higher timeouts (see \eg\ \cite{BFHH17}). When looking at the time needed to decide instances, the only tool able to compete is \textsc{Bfc}, a state-of-the-art coverability checker tailored to coverable instances.

%% \input{benchmark-figs/fig-coverability.tex}

%% On uncoverable instances, the merit of using pruning and relaxations to discard candidate markings is clear: The only tool that can compete is \textsc{ICover},
%% which also uses these two techniques. Their impact is also exhibited in the similar shapes of the graphs of \textsc{ICover} and \textsc{FastForward} for uncoverable instances.
%% On all but two uncoverable instances, \textsc{FastForward} establishes uncoverability either after pruning, or after calculating $d_{\Q}$ from the initial marking. This also explains why there is almost no difference between \astar\ and GBFS.
%% Of the two remaining instances, one is small enough that the reachability graph is fully explored without finding the target.
%% On the other instance, $d_{\Q}$ considers that the initial marking can reach the target. However, after a few steps, both \astar\ and GBFS establish a frontier where $d_{\Q}$ evaluates to $\infty$, which proves uncoverability.

%% \textsc{FastForward} decides the most instances, with a total of 152/176 instances. \textsc{ICover} decides the second most instances, totalling 144/176 instances. As the graphs show, neither tool subsumes the other: Both tools together solve 166/176 instances. 
%% The remaining tools are vastly outperformed by either of these two.

%\paragraph*{Witnesses length.}

%\input{benchmark-figs/fig-paths.tex}




==> ssec-liveness.tex <==
\subsection{Liveness checking}

Lastly, we used four benchmark suites for liveness checking collected
by \textsc{Petrinizer}~\cite{EM15}. For three suites, we check for
\emph{termination}, \ie\ whether there is an infinite execution:
\begin{itemize}
\item \emph{IBM}: 124 nonterminating and 1264 terminating instances modeling business processes~\cite{FFJKLVW09};
  
\item \emph{soter}: 17 nonterminating and 33 terminating instances
  arising from the verification of Erlang concurrent programs (one of
  the suites used for coverability);

\item \emph{Literature}: 5 terminating instances arising from the
  literature on termination and liveness analysis (used by the tool
  \textsc{Petrinizer}).
\end{itemize}

The last suite contains models for 6 classical algorithms parameterized by the number of processes ranging from $2$ to $6$, for a total of 30 instances.
Four of these algorithms are concerned with mutual exclusion, and for these we check for starvation freedom of the first process.
Of the remaining two algorithms, one is a snapshot algorithm, for which we check that a snapshot is taken infinitely often; and the other is a leader election algorithm, for which we check that a leader is elected infinitely often. All instances of the last benchmark suite satisfy their respective property.

There are two caveats here. The first is that \textsc{LoLA} does not directly support the liveness properties we are interested in.
However, instances of the \emph{IBM} suite have been converted by~\cite{EM15} into reachability queries that \textsc{LoLA} can handle.
For the other instances, such a conversion does not exist, so \textsc{LoLA} could only run on the 1388 instances from the \emph{IBM} suite. Due to the converted setting, the execution time of \textsc{LoLA} is therefore not fully comparable to that of the other tools.
The second caveat is that \textsc{Petrinizer} cannot decide instances that do not satisfy termination/liveness.
However, these only make up around a tenth of the total instances.
Despite these caveats, we still include both tools, since the \emph{IBM}  suite and terminating instances make up the majority of the instances.
Further, there are fewer tools that support this setting compared to coverability and reachability.

\input{benchmark-figs/fig-liveness.tex}

\Cref{fig:liveness-benchmark} shows the results of the evaluation. \textsc{FastForward} and \textsc{Petrinizer} perform better than \textsc{LoLA} on instances that satisfy termination/liveness.
The main reason for this is that on all of these instances, the first call to the heuristic made by \textsc{FastForward} suffices to conclude that no certificate exists.
Since \textsc{Petrinizer} uses an approach based on so-called \emph{T-surinvariants} that shares many characteristics with our approach on terminating/live instances, it comes as no surprise that the performance of the tools is almost identical. There is a single instance where \textsc{FastForward} runs out of memory but which is decided by \textsc{Petrinizer}.

On nonterminating instances, \textsc{LoLA} decides more instances than \textsc{FastForward}.
Additionally, it is generally faster, which may suggest that the performance of our approach does not translate to this setting.
Further, the \emph{IBM} benchmark suite contains only 1-safe Petri nets, so with finite reachability graphs,
which \textsc{LoLA} supports very well. 
Overall, \textsc{FastForward} decides the most instances, with a total of 1394/1473 instances, with \textsc{LoLA} in second place with 1337/1473 instances, followed by \textsc{Petrinizer} with 1310/1473 instances.

Note that \textsc{LoLA} could only participate on 1388 of the total of 1473 instances. It is reasonable to expect that if it participated on all instances, \textsc{LoLA} could decide as many or more instances as \textsc{FastForward}.


==> ssec-reachability.tex <==
\subsection{Reachability}

\paragraph*{Instances proven.}

\Cref{fig:reachability} depicts the number of instances found
reachable within the time limit. The left-hand and right-hand side
respectively correspond to the \emph{sypet} suite and the instances
obtained from random walks.\michael{Will we have data for GBFS?}\philip{it's not planned yet, but we can get it if we want it}

\input{benchmark-figs/fig-reachability}

The instances from \emph{sypet} are notable for two reasons.  First,
they typically have a short witness: the minimal one has length at
most 5 on all 30 instances, and lengths 1 or 2 on 14
instances. Additionally, the branching factor is typically very large:
Each instance has between 23 and 187 unguarded transitions. Since
these are always enabled, this gives a lower bound on the branching
factor. Most markings tend to enable guarded transitions, so the
average branching factor is even larger. The branching factor on the
initial marking ranges from 30 to 300.\michael{Is this still relevant
  without the structural distance?}\footnote{Chess and Go respectively
  have an average branching factor of $\sim$35 and
  $\sim$350~\cite{RN09}.}

%% A comparison between greedy best-first search with $\mathcal{D}_\text{struct}$ and \astar\ with $\mathcal{D}_{\Q}$ shows that the former is faster on most instances. However, it is vastly outperformed by \astar\ on a few instances.
%% An explanation is provided by the aforementioned large branching factor and short paths, and how these emphasize the characteristics of the different approaches.
%% Note that the structural abstraction can be precomputed in linear time in the size of the {P}etri net. On the other hand, \astar\ requires computing the heuristic to be evaluated on each successor before the next node is chosen for expansion, and $\mathcal{D}_{\Q}$ is more expensive.
%% It thus is at a slight disadvantage on instances where a shortest witness is so short that it is found rather quickly even with the coarse structural distance.
%% Its advantage is on the instances where the length of a shortest witness is at the upper end of the range. There, the large branching factor comes into play and a search algorithm must more aggressively discard parts of the search space.
%% For both instances where greedy best-first search with $\mathcal{D}_\text{struct}$ times out, shortest paths have length 5.

